Deep Reinforcement Learning for Safe Landing Site Selection with Concurrent Consideration of Divert Maneuvers

This research proposes a new integrated framework for identifying safe landing locations and planning in-flight divert maneuvers. The state-of-the-art algorithms for landing zone selection utilize local terrain features such as slopes and roughness to judge the safety and priority of the landing point. However, when there are additional chances of observation and diverting in the future, these algorithms are not able to evaluate the safety of the decision itself to target the selected landing point considering the overall descent trajectory. In response to this challenge, we propose a reinforcement learning framework that optimizes a landing site selection strategy concurrently with a guidance and control strategy to the target landing site. The trained agent could evaluate and select landing sites with explicit consideration of the terrain features, quality of future observations, and control to achieve a safe and efficient landing trajectory at a system-level. The proposed framework was able to achieve 94.8 $\%$ of successful landing in highly challenging landing sites where over 80$\%$ of the area around the initial target lading point is hazardous, by effectively updating the target landing site and feedback control gain during descent.

==> Conclusion.tex <==
\section{Conclusion}
Some AAS meetings are co-sponsored with the American Institute of Aeronautics and Astronautics (AIAA). When your paper number starts with ``AAS'', or when the conference is described as a joint ``AAS/AIAA'' meeting with the AAS listed first, this AAS conference proceedings format shall be used.

Your final manuscript should be camera-ready as submitted --- free from technical, typographical, and formatting errors. Manuscripts not suitable for publication are omitted from the final proceedings.


==> Nomenlecture.tex <==
\section{Notation}
\begin{tabular}{r l}
	$a$ & a real number \\
	$b$ &  the square root of $a$ \\
\end{tabular} \\

If extensive use of mathematical symbols requires a table of notation, that table may appear here. Where the first mathematical symbol is introduced, a footnote should direct the attention of the reader to this table.\footnote{The footnote symbols are a standard sequence: $\ast$, $\dagger$, $\ddag$, \emph{etc}. This sequence of footnote symbols should restart with each new page.}  The notation table should be simple and reasonably consistent with the standards of modern technical journals, as illustrated above. The notation table does not need its own caption like an ordinary table, since the section heading serves this purpose. The notation section is optional.
